AgentOccam: A Simple Yet Strong Baseline for LLM-Based Web Agents

Autonomy via agents using large language models (LLMs) for personalized, standardized tasks boosts human efficiency. Automating web tasks (like booking hotels within a budget) is increasingly sought after. Fulfilling practical needs, the web agent also serves as an important proof-of-concept example for various agent grounding scenarios, with its success promising advancements in many future applications. Prior research often handcrafts web agent strategies (e.g., prompting templates, multi-agent systems, search methods, etc.) and the corresponding in-context examples, which may not generalize well across all real-world scenarios. On the other hand, there has been limited study on the misalignment between a web agent's observation/action representation and the pre-training data of the LLM it's based on. This discrepancy is especially notable when LLMs are primarily trained for language completion rather than tasks involving embodied navigation actions and symbolic web elements. Our study enhances an LLM-based web agent by simply refining its observation and action space to better align with the LLM's capabilities. This approach enables our base agent to significantly outperform previous methods on a wide variety of web tasks. Specifically, on WebArena, a benchmark featuring general-purpose web interaction tasks, our agent AgentOccam surpasses the previous state-of-the-art and concurrent work by 9.8 (+29.4%) and 5.9 (+15.8%) absolute points respectively, and boosts the success rate by 26.6 points (+161%) over similar plain web agents with its observation and action space alignment. We achieve this without using in-context examples, new agent roles, online feedback or search strategies. AgentOccam's simple design highlights LLMs' impressive zero-shot performance on web tasks, and underlines the critical role of carefully tuning observation and action spaces for LLM-based agents.

==> Tables/action_statistics_color.tex <==
\begin{table}[t]
\centering
\caption{Action statistics for the ablation study of \codename's components. Each number in the table represents the frequency of an action across all the tasks within the experiment setting.}
\label{table:action_statistics}
{\scriptsize
\begin{tabular}{c|c|c|c|c|c|c|c|c|c}
\hline
Exp. & noop & click & hover & type & press & scroll & tab\_focus & new\_tab & tab\_close \\ \hline
Vanilla; IAE-0 & \valuecolor{0}{339.0}{0.0} & \valuecolor{2328}{7119.0}{0.0} & \valuecolor{126}{511.0}{126.0} & \valuecolor{1024}{2531.0}{112.0} & \valuecolor{7}{801.0}{7.0} & \valuecolor{132}{370.0}{23.0} & \valuecolor{0}{34.0}{0.0} & \valuecolor{20}{47.0}{20.0} & 0          \\
IAE-1 & - & \valuecolor{7119}{7119.0}{0.0} & - & \valuecolor{2531}{2531.0}{112.0} & - & \valuecolor{370}{370.0}{23.0} & - & - & -          \\
IAE-2 & - & \valuecolor{7033}{7119.0}{0.0} & - & \valuecolor{2390}{2531.0}{112.0} & - & - & - & - & -          \\
IAE-3 & - & \valuecolor{6890}{7119.0}{0.0} & - & \valuecolor{2040}{2531.0}{112.0} & - & - & - & - & -          \\
IAE-4 & - & \valuecolor{4625}{7119.0}{0.0} & - & \valuecolor{1286}{2531.0}{112.0} & - & - & - & - & -          \\
\codename & - & \valuecolor{4720}{7119.0}{0.0} & - & \valuecolor{1159}{2531.0}{112.0} & - & - & - & - & -          \\ \hline
 & go\_back & go\_forward & goto & note & stop & go\_home & branch & prune & \\ \hline
Vanilla; IAE-0 & \valuecolor{71}{339.0}{0.0} & \valuecolor{0}{7119.0}{0.0} & \valuecolor{511}{511.0}{126.0} & - & - & - & - & - & \\
IAE-1 & \valuecolor{52}{339.0}{0.0} & - & - & \valuecolor{194}{2531.0}{112.0} & \valuecolor{512}{801.0}{7.0} & \valuecolor{36}{370.0}{23.0} & - & - & \\
IAE-2 & \valuecolor{100}{339.0}{0.0} & - & - & \valuecolor{219}{2531.0}{112.0} & \valuecolor{536}{801.0}{7.0} & \valuecolor{42}{370.0}{23.0} & - & - & \\
IAE-3 & \valuecolor{56}{339.0}{0.0} & - & - & \valuecolor{201}{2531.0}{112.0} & \valuecolor{571}{801.0}{7.0} & \valuecolor{23}{370.0}{23.0} & - & - & \\
IAE-4 & \valuecolor{94}{339.0}{0.0} & - & - & \valuecolor{112}{2531.0}{112.0} & \valuecolor{801}{801.0}{7.0} & \valuecolor{54}{370.0}{23.0} & - & - & \\
\codename & \valuecolor{339}{339.0}{0.0} & - & - & \valuecolor{197}{2531.0}{112.0} & \valuecolor{769}{801.0}{7.0} & \valuecolor{42}{370.0}{23.0} & \valuecolor{34}{34.0}{0.0} & \valuecolor{47}{47.0}{20.0} & \\ \hline
\end{tabular}}
\end{table}

==> Tables/comparison_with_baselines.tex <==
\begin{table}[t]
\centering
\begin{tabular}{c|c|c}
\hline
Approach                   & Model       & WebArena Success Rate (\%) \\ \hline
SteP                       & GPT-4-Turbo & 33.5                       \\
AWM                        & GPT-4       & 35.5                       \\
WebPilot                   & GPT-4       & 37.2                       \\
Odysseus                   & GPT-4-Turbo & 43.1                       \\
Odysseus + SteP Strategies & GPT-4-Turbo & 41.13*                     \\ \hline
\end{tabular}
\end{table}
